Finch: Sparse and Structured Tensor Programming with Control Flow

From FORTRAN to NumPy, tensors have revolutionized how we express computation. However, tensors in these, and almost all prominent systems, can only handle dense rectilinear integer grids. Real world tensors often contain underlying structure, such as sparsity, runs of repeated values, or symmetry. Support for structured data is fragmented and incomplete. Existing frameworks limit the tensor structures and program control flow they support to better simplify the problem. In this work, we propose a new programming language, Finch, which supports both flexible control flow and diverse data structures. Finch facilitates a programming model which resolves the challenges of computing over structured tensors by combining control flow and data structures into a common representation where they can be co-optimized. Finch automatically specializes control flow to data so that performance engineers can focus on experimenting with many algorithms. Finch supports a familiar programming language of loops, statements, ifs, breaks, etc., over a wide variety of tensor structures, such as sparsity, run-length-encoding, symmetry, triangles, padding, or blocks. Finch reliably utilizes the key properties of structure, such as structural zeros, repeated values, or clustered non-zeros. We show that this leads to dramatic speedups in operations such as SpMV and SpGEMM, image processing, and graph analytics.

==> sections/cut.tex <==
\HIDE{From FORTRAN to NumPy, arrays have revolutionized how we express computation.  Tensors are the highest-performing datastructure with a long history of investment and innovation, from hardware support to compiler technology.  However, arrays can only handle dense rectilinear integer grids. Real world arrays often contain underlying structure, such as sparsity, runs of repeated values, or symmetry. We describe a compiler, Finch, which adapts existing programs and interfaces to the structure and sparsity of the inputs. Finch enables programmers to capture complex, real-world data scenarios with the same productivity they expect from dense arrays. Our approach enables new loop optimizations across multiple domains, unifying techniques such as sparse tensors, databases, and lossless compression. }

\HIDE{
Of the nearly 44 zettabytes of data humans have gathered to date, most of it is collected, processed, and stored as multi-dimensional arrays.
Multi-dimensional arrays are the most prominent data type from the first programming language FORTRAN to modern Numpy.
Furthermore, multi-dimensional arrays are the highest-performing data structure with a long history of investment and innovation, from hardware support to compiler technology.
Tensors in these, and almost all prominent systems, can only handle dense rectilinear integer grids.
However, a large portion of the data, either obtained from nature or generated by humans, have structure.  

Over the years compiler researchers have valiantly attempted to put sparse tensor algebra on the same compiler transformation and code generation footing as dense tensor algebra and array codes. So far this has failed in both scope of the ambition and execution of comparable features.  Real world data have structure beyond sparsity including runs of repeated values, dense blocks or diagonals, ragged edges, or symmetry. 
Thus, focusing only on sparsity limits the scope needed to handle the staggering variety of data. Second, the arrays and loops abstraction introduced in FORTRAN supports lot more complex control flow not supported by einsum based modern sparse array compilers. For example, complex control flow such as conditional branches and early exits are needed for many important computations such as graph analytics. 
 
In this paper, we describe a compiler, Finch,
which adapts existing programs and interfaces to the structure and sparsity of the inputs. Finch enables
programmers to capture real-world scenarios with structured data and complex control flow with the same productivity they expect from dense arrays. Our approach enables new loop optimizations across multiple domains, unifying techniques in areas such as
sparse tensors, databases, and lossless compression.
We hope to truly bring tensor algebra on structured data to the same compiler transformation and code generation footing as dense tensor algebra and array codes.}
% \teo{
% Due to this fine grained mixing of control flow and data structures, we dub a new programming model for Finch: ``Fine Grained Data Structure Driven Tensor Programming''.
% %
% Finch supports \textit{both} flexible programming constructs and diverse data structures. 
% %
% Finch supports a similar programming language of loops, statements, if conditions, breaks, etc, over a wide variety of array structures, such as sparsity, run-length-encoding, symmetry, triangles, padding, or blocks.
% %
% The Finch compiler uses the structure
% of the data to generate efficient implementations of these programs by predictably converting the control flow into the same representation as the data, Looplets~\cite{ahrens_looplets_2023}.}


%% Many variations of this problem.
%By combining many data structures and control flows into a single language, a performance engineer could use a sufficiently predicable and fine grained compiler to find efficient programs.
%
%We dub this model, ``Datastructure-driven Tensor Programming'' in which the programmer specifies the structure of the data separately from the program, but then can reasonably iterate on the two with a compiler that predicable combines them, leading to efficient code eventually.
%
%(Note quite sure how much comes after this)
%We should say the predicability is generating only the non-zeros! We leverage the intiial stuff of Finch to say we will in order generate the code that only grabs the non-zeros, modified in certain ways based on the fine grained ordering of computation)
%(Use the below comment as an example - where the old paragraph talked about merging two lists.)


%In this work, we propose a new programming model we call ``Datastructure-driven Tensor Programming'' in which the programmer specifies the structure of the data separately from the program, and the compiler uses these two descriptions to generate efficient code.\saman{Is this new? TACO did something similar?} In this model, performance engineers can more efficiently search the
%complex landscape of programs and datastructures to find the best implementation. In this programming model, we can express certain concepts in programs, and others in data. For example, if we wish to merge two sorted lists, we express this as two sparse vectors which are true whenever the list contains the key in question, and we iterate over the \textit{entire} space of keys, writing to the output list whenever either of the vectors are true.
%While the order in which we iterate over the data is expressed in the program, which datapoints are of interest and how to find them is expressed in the data.


%Taichi enriches single static assignment form with specialized instruction for accessing a single sparse structure drawn from a particular class, which is why it supports the most control flow for a single sparse structure~\cite{hu_taichi_2019}.
%
%Furthermore, the limits and advantages of a DSL can be traced to the specific coupling of a program's control flow with the data structure: many new TACO features required modifying algorithms that worked with TACO's merge lattices and Tiramisu can express programs that Halide can't because Tiramisu uses a polyhedral model as opposed to a model built on iterating over regular grids~\cite{kjolstad_tensor_2017, henry_compilation_2021, senanayake2020sparse, baghdadi2019tiramisu}.
%
%In this work, we will choose  a new representation of a program's data structures and control flows that covers a wide range of programs.
%
%However, simply combining a large variety of structured data with a large variety of programs does not necessarily yield a performance advantages.
%
%After all previous implementations choose to tightly couple to a specific data structure in part to ensure the data structures are iterated over efficiently.
%
%To find and produce efficient programs for structured data, we must overcome two challenges that occur when we intersect complex control flow with structured data:

%before introducing this, we must discuss performance: if we want to also produce efficient code for structured data, we face two challenges.



%build on some conception of an iteration space: TACO has merge lattices, Polyhedral compilers rely on the polyhedral model, Halide and Corra uses rectangular intervals, and so on.
%
%And we believe the limitations of these systems can be traced back to their specific conceptions.} \willow{I agree with what this sentence is saying, but I'm concerned that the sentiment is unclear, because here it may seem like we say "iteration space bad" and later say "iteration space good". Can we perhaps adjust here to say may of these special purpose compilers use overly restrictive models of the iteration space of the program, but that Finch is good because it uses general control flow to express a wider variety of iteration spaces. At a high level, we need to define "iteration space" or "control flow" or "Looplets" if we want to use them in the intro, and depending on how much we want to use these words we may want to avoid them here.}
%
% \teo{For example, each modification to expressions that TACO could support required modifying the merge lattice algorithms\cite{kjolstad_tensor_2017, henry_compilation_2021, senanayake2020sparse} and several programs could not be supported in Halide, but could be in Tiramisu due to the limitations of a rectangular iteration space~\cite{baghdadi2019tiramisu}.
% %
% And many iteration space concepts simply don't allow for skipping work that isn't simply the complement of an interval.
% %
% In our work, we will show how we can use Looplets as our main tool to manage the iteration spaces of our computations and data structures.
% %
% However, to support as many data structures and iteration spaces as is implied above, we face two challenges if we want to also produce efficient code over structured data.
% }
%We see two main challenges to writing efficient code over structured data.
\teo{How about:
A Looplet based level-format abstraction.
%
Although many systems (TACO, Taichi, SPF, Ebb)~\cite{chou2018format,  hu_taichi_2019, strout2018sparse, bernstein2016ebb} features a flexible data structure description language for array-like computations, we show that we can describe more level formats than any other by a level format abstraction designed to target Looplets in the context of an array programming language with fine-grained control flow. 
%
The first such set of formats to efficiently capture banded,
triangular, run-length-encoded, or sparse datasets, and any combination thereof.
}


with key level formats that completely capture the main structural properties of data. for expressing the structure of data
hierarchically.\saman{level formats were done in TACO.} The first such set of formats to efficiently capture banded,
triangular, run-length-encoded, or sparse datasets, and any combination thereof.

%
\teo{
The Finch language offers extensible abstractions for elements of control flow (conditionals and indexing expressions) that the Finch compiler predictably converts into the same structured representation used to describe arrays.
%
By controlling how control flow is lowered into this representation, a programmer can control how structured data is combined with control flow to produce a single control flow, the program.
%
We observe that this strategy naturally extends the dense solution.
}
\teo{I think we can back it up in two ways:
1. We need to modify the semantics to focus when on when things are converted into Looplets
2. We need to highlight the specifics in the case studies: in particular, the blur and the symmetric operations. If we do triangle counting or something like that, we could maybe talk about that a bit.
}
\teo{
\item Extensibility of the language and compiler with respect to data structures and control flow: (Maybe put stuff about the data structure extensibility here?)
}

   
\scriptsize
\noindent % This ensures the minipages fill the page width
\begin{minipage}{0.4\linewidth}
\begin{align*}
    \finchliteral(val \in \mathbb{V}) &:= \text{\mintinline{julia}{val}} \\
    \finchvalue(ex \in \mathbb{S}, type \in \mathbb{T}) &:= \text{\mintinline{julia}{ex :: type}} \\
    \finchtensor(name \in \mathbb{S}) &:= \text{\mintinline{julia}{name}} \\
    \finchindex(name \in \mathbb{S}) &:= \text{\mintinline{julia}{name}} \\
    \finchvar(name \in \mathbb{S}) &:= \text{\mintinline{julia}{name}} \\
    \finchextent(a \in E, b \in E) &:= \text{\mintinline{julia}{a : b}} \\
    \finchcall(f \in E, args\ldots \in E) &:= \text{\mintinline{julia}{f(args...)}} \\
    \finchaccess(tns \in T, idxs\ldots \in E) &:= \text{\mintinline{julia}{tns[idxs...]}} \\
    \finchfreeze(tns \in T) &:= \text{\mintinline{julia}{@freeze(tns)}} \\
    \finchthaw(tns \in T) &:= \text{\mintinline{julia}{@thaw(tns)}} \\
    \finchmode(tns \in T) &:= \text{\mintinline{julia}{@mode(tns)}} \\
\end{align*}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\begin{align*}
    \mathbb{V} &:= \text{the set of all values.} \\
    \mathbb{S} &:= \text{the set of all symbols.} \\
    \mathbb{T} &:= \text{the set of all types.} \\
    I &:= \finchindex \\
    A &:= \finchaccess \\
    V &:= \finchvar \\
    T &:= \finchtensor \\
    E &:= \finchliteral \mid \finchvalue \mid \finchindex \\
        &\quad \mid \finchvar \mid \finchextent \mid \finchcall \mid \finchaccess \\
    S &:= \finchassign \mid \finchloop \mid \finchdefine \\
        &\quad \mid \finchsieve \mid \finchblock \\
\end{align*}
\end{minipage}%
\begin{align*}
    \finchdeclare(tns \in T, init \in E, dims\ldots \in E) &:= \text{\mintinline{julia}{tns .= init(dims...)}} \\
    \finchassign(lhs \in A, op \in E, rhs \in E) &:= \text{\mintinline{julia}{lhs <<op>>= rhs}} \\
    \finchloop(idx \in I, range \in E, body \in S) &:= \text{\mintinline{julia}{for idx = range; body end}} \\
    \finchdefine(var \in V, val \in E, body \in S) &:= \text{\mintinline{julia}{let var = val; body end}} \\
    \finchsieve(cond \in E, body \in S) &:= \text{\mintinline{julia}{if cond; body end}} \\
    \finchblock(bodies\ldots \in S) &:= \text{\mintinline{julia}{begin; bodies... end}}
\end{align*}

==> sections/eval/api.tex <==
\subsection{Implementing NumPy's Array API in Finch}
In the past decade, the adoption of the Python Array API \cite{harris_array_2020} has allowed for a proliferation tensor programming systems, but existing implementations of this and similar APIs for structured data suffer from either incompleteness or inefficiency.
%
These APIs have hundreds of required functions, from mapreduce to slicing and windowing. 
%
Compilers with simpler interfaces (such as TACO's simple Einsum) need a massive amount of glue code outside of the normal compilation path to support the full API, leading to a large implementation burden.
%
As the API's were designed for only one structure (Dense), the burden only grows with the introduction of as additional structures such as sparsity, as these structures interact with the complex interface and with each other.
%
%In order to reduce the complexity of interactions between different formats, they're either limited to vectors and matrices or only support tabular representations.
%
Further, implementing each operation on its own is insufficient. Operator fusion is required to avoid asymptotic performance degradation on sparse kernels, as we show in Figure~\ref{fig:fusion}.
%
A flexible compiler like Finch, which can produce efficient code for arbitrary operations between inputs in a wide variety of formats, is the missing piece needed to implement the full tensor API for structured data with competitive performance.
%
To handle the expansiveness of the Array API while preserving opportunities for fusion and whole workflow optimization, we pursued a lazy evaluation strategy mediated by a high-level query language.
%
This is implemented by 1) Finch Logic, a minimal, high-level language for expressing tensor operations and 2) the Physical Interpreter, which executes Finch Logic as a sequence of Finch programs.

%Add a list of all of the functions we currently support, and claim that other frameworks cannot do the same.
%Masks and wrapper tensors -> needed to implement indexing and slicing
%Custom operators -> needed to implement argmin, norm, ifelse, and other "weird" operations

%Add back the nice stuff that kyle cut
%Languages like TACO that are very simple can be trivially incorporated as a library function interface into python.
%However, Finch provides many other features and control flow than TACO, that are more challenging to integrate.
%Instead of pushing Finch literally into the hands of python users, we are using their language to describe functions, similar to pytorch.


%There is a gap between the expressiveness of the purely declarative Array API and the Finch language which defines both the output and the algorithm. The naive approach to solving this would be to explicitly define a mapping from each function in the API to a Finch program which eagerly produces the output. This approach results in a simple translation procedure but misses crucial opportunities for optimization across a chain of function calls and needlessly materializes large intermediate results. To avoid this, we have implemented a lazy evaluation approach that collects API calls and then computes output when requested by the user.

\begin{wrapfigure}{R}{0.57\linewidth}
  \scriptsize
  \vspace{-12pt}
\begin{minted}{julia}
  EXPR := table(TENSOR, FIELDS...) |           #TENSOR is a tensor value
    ALIAS | FIELD | mapjoin(OP, EXPRS...) |    #OP is a function
    aggregate(OP, INIT, EXPR, FIELDS...) |     #INIT is an initial value
    reorder(EXPR, FIELDS...) |                 #FIELD is a name for an index
    relabel(EXPR, FIELDS...) |                 #ALIAS is a name for a tensor
    reformat(TENSOR, EXPR)                       PLAN := plan(QUERIES...)
                                                QUERY := query(ALIAS, EXPR)
\end{minted}
\vspace{-12pt}
\caption{\footnotesize Finch Logic Syntax. }\label{fig:finch_logic_syntax}
\vspace{-12pt}
\end{wrapfigure}
\begin{figure}[b]
\begin{minted}{python}
  sum(A, dims=2) = aggregate(+, relabel(A, i_1, ..., i_d), i_2)
  matmul(A, dims=2) = aggregate(+, mapjoin(*, relabel(A, i, j), relabel(B, j, k)))
  argmin(A) = aggregate(minby, (Inf, len(A)), mapjoin(tuple, relabel(A, i), i), i)
  norm2(A) = aggregate(scaled_plus, (0, 0), mapjoin(tuple, mapjoin(sign, A), mapjoin(abs, A)), fields(A)...)
  where(C, A, B) = mapjoin(ifelse, relabel(C, i), relabel(A, i), relabel(B, i))
  slice(A, i:j) = table(WindowedArray(A, i:j), k)
  cat(A, B) = mapjoin(coalesce, table(PermissiveArray(A), i), table(OffsetArray(B, length(A)), i))
\end{minted}
\vspace{-12pt}
\caption{\footnotesize Implementations of a few common functions in Finch Logic. Here, \texttt{minby(x, y)} compares \texttt{x[1]} and \texttt{y[1]} and returns the smaller \texttt{x} or \texttt{y}. \texttt{scaled\_plus} rescales whichever argument is smaller, then adds the values with the same scale. \texttt{ifelse(c, a, b)} returns \texttt{a} when \texttt{c} is true,  \texttt{b} otherwise. Finch can understand declared properties and rewrite rules for all of these functions and types, extending these algorithms to operate on structured arguments.} \label{fig:api_extensible}
\vspace{-18pt}
\end{figure}
\subsubsection{Finch Logic and the Physical Interpreter}
Finch Logic is used as a common representation to implement and fuse the operations in the Array API.
%
The syntax is designed to be minimal and expressive, taking inspiration from relational algebra with the goal of being able to express most of the operations in the Array API.

\paragraph{Finch Logic}
The syntax of Finch Logic is described in Figure~\ref{fig:finch_logic_syntax}.
%
Our \texttt{mapjoin} represents pointwise application, while \texttt{aggregate} represents reductions.
%
We name the result of each computation with \texttt{query}, and join several expressions in a \texttt{plan}.
%
\texttt{reorder} reorders the indices while \texttt{relabel} relabels them.
%
\texttt{reformat} hints at materialization into its argument.

Finch's support for arbitrary user-defined functions allows us to support complex operations such as \mintinline{python}{argmin}, \mintinline{python}{norm}, and \mintinline{python}{where}, all over structured data. Finch's support for wrapper tensors allows us to express indexing operations. These situations are shown in Figure~\ref{fig:api_extensible}.
\begin{figure}

\end{figure}

\paragraph{Heuristic Optimization}
Once we express our operation in Finch Logic, we use a quick heuristic to fuse the expressions. 
%
We heuristically split nested \texttt{aggregate} queries into separate queries, and fuse all of the \texttt{mapjoin}s into corresponding \texttt{aggregate}s.
%
We then heuristically choose a loop order for each query with \texttt{reorder} nodes, and introduce separate \texttt{query} nodes to transpose so that the resulting expressions are concordant.
%
Our heuristic assigns a format to each output by recursively evaluating the properties of structure (sparsity, repetition, etc.) and checking whether they are preserved under the operation in question.

%The expression fragment takes inspiration from relational algebra while incorporating an ordering on the dimensions of a tensor. This means that operators take in a set of indexed tensors and output an indexed tensor. Conceptually, an indexed tensor can be thought of as a relation with an ordering on the index attributes and a separate value attribute, and we include the $\finchreorder$ operator to manipulate this order. To express materialization, reuse of common sub-expressions, and multiple outputs, we define $\finchquery$ and $\finchplan$. A $\finchquery$ assigns the output of an expression to a name. We use this to denote that we materialize an expression. Later queries can access the result of earlier queries through the $\finchalias$ operator, allowing multiple queries to benefit from a shared computation. A plan is a sequence of queries and outputs a set of tensors. 
%This ordering is necessary for two reasons 1) the outputs of a function in the Array API must match a defined order on the dimensions based on the order of the inputs' dimensions 2) to benefit from concordant iteration we must ensure that the operands to a mapjoin have compatible index orders.

%\begin{align*}
%    \footnotesize \finchplan(queries..., names...) \quad\quad\quad \finchquery(name, expr) \quad\quad\quad \finchreorder(expr, idxs...)\\
%     \footnotesize \finchrelabel(expr, idxs...) \quad\quad\quad \finchreformat(expr, format) \quad\quad\quad \finchmapjoin(op, exprs...) \\
%    \footnotesize\finchaggregate(op, expr)\quad\quad\quad\quad \finchtable(tns, idxs...)  \quad\quad\quad\quad\quad\quad \finchalias(name) \quad\quad\\
%     \footnotesize expr:= \finchreorder | \finchrelabel | \finchreformat |\finchmapjoin | \finchaggregate | \finchtable | \finchalias \quad\quad
%\end{align*}

%We now describe how to define a few example functions from the API in this language. Due to the flexibility of Finch, we can use the custom operators $minby(x,y)$ (which compares $x[1]$ and $y[1]$ and returns the smaller $x$ or $y$) and $tuple(x, y)$ (which returns the tuple $(x,y)$), and we can treat an index as a scalar to implement $argmin$. For conciseness, we omit the outer $\finchplan(\finchquery(out,...),out)$.
%\begin{align*}
%&\footnotesize \text{sum}(M, dims=[2]) \rightarrow \finchaggregate(+,\finchrelabel(M, i_1,\ldots,i_d), i_2)\\
%&\footnotesize \text{matmul}(A, B) \rightarrow \finchaggregate(+,\finchmapjoin(*, \finchrelabel(A, i, j), \finchrelabel(B, j, k)), j)\\
%&\footnotesize \text{argmin}(A, dims=[2]) \rightarrow \finchaggregate(minby,\finchmapjoin(tuple, \finchrelabel(A, i_1,\ldots,i_d), \finchtable(i_2)), i_2)
%\end{align*}

%Notably, these plans do not specify important details about the computation such as the format of intermediates and the order of the loops. In the following discussion, we provide sensible heuristics and show that they provide good performance on important kernels. However, for larger or more complex programs, it would be important to apply a cost-based optimization strategy which we leave for future work.

%\paragraph{Execution}
%\subsubsection{Standardizing \& Heuristic Optimization}
%Before a plan in Finch Logic can be interpreted, it must be converted to a standard form which resolves ambiguity about loop ordering and output formatting. The semantically important requirements of this standard form are 1) all inputs (i.e. tables and alias operators) in a query's RHS must conform to a common ordering of the indices 2) the outermost operator of each query's RHS must be a reformat 3) the expression within the reformat must be a pointwise expression, optionally wrapped in an aggregate operator. The former allows the interpreter to identify the loop order for each kernel. The second determines the output format for each intermediate. The last one guarantees that the innermost expression can be computed as a single kernel. To achieve this: 1) a concordization pass examines each query, heuristically selects a loop order, and transposes inputs which don't match that order 2) a formatting pass selects a level format for each output index based on the formats of the inputs and whether the loop order requires random writes. In future work, these heuristics could be improved with cost-based optimization similar to query optimization in the database setting.

% based on a heuristic which loops over intersecting variables first.

\paragraph{Finch Interpreter} 
Once the program is in a standard form where each \texttt{query} has a specified format with \texttt{reformat} and at most one \texttt{aggregate}, the Finch Interpreter executes each query, in order, through a straightforward lowering process.
%
%Each result is assigned to the corresponding alias the .
% The output format is identified by unpacking the outer $\finchreformat$ statement. Next, the inner expression of the is unpacked to identify the $\finchaggregate$ operator and extract the pointwise expression. At this point, any aliases to the result of previous queries are replaced with an access to the actual result. Lastly, the concordant loop order is identified and instantiated. The lowered query is then compiled and executed with the Finch compiler, and the result is assigned to $name$ before proceeding to the next query. 


\subsubsection{Evaluation}
To demonstrate the performance of our tensor implementation, we evaluate it on 1) triangle counting 2) SDDMM 3) and element-wise operations. Further, we compare against DuckDB as a state of the art system which implements a form of kernel fusion through pipelined query execution. To do this, we express each of these kernels as a single select, join, groupby query. For the element-wise case, we provide an unfused Finch method to show the impact of fusion. For triangle counting, we use the same set of graph matrices as in Figure~\ref{fig:graph_result}. For SDDMM, we use this set of graph matrices for the sparse matrix, and we produce random dense matrices with embedding dimension 25. Lastly, for the elementwise operations, we use uniformly sparse matrices with dimension 10000 by 10000. A/B have sparsity $.1$, and we vary the sparsity of C in the X axis.

%we evaluate it on a series of kernels which benefit from the kind of kernel fusion that it automatically applies

Across all three of these kernels, we see that the high level interface for Finch provides a major improvement over DuckDB, ranging from $1.2x-28x$. For triangle counting and SDDMM, this improvement stems from Finch's efficient intersection of the nonzero indices as opposed to DuckDB's use of binary join plans\footnote{This matches with findings in the database literature showing that worst-case optimal joins (which are very similar to our kernel execution) are more efficient than binary joins for these queries \cite{wang_free_2023}.}. For element-wise operations, this improvement stems from Finch's better handling of expressions which combine index intersection and union and its compressed data representation.

\begin{figure}
  \centering % Centers the figure block in the text area
  % First minipage for the first image
  \begin{minipage}[t]{0.32\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figures/triangle_count_speedup_over_duckdb.png}
    \vspace{0pt}
  \end{minipage}%
  % Second minipage for the second image
  \begin{minipage}[t]{0.32\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figures/sddmm_speedup_over_duckdb.png}
    \vspace{0pt}
  \end{minipage}%
  % Third minipage for the third image
  \begin{minipage}[t]{0.36\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figures/elementwise_speedup_over_duckdb.png}
    \vspace{0pt}
  \end{minipage}

  \vspace{-24pt}
  \caption{Performance of Finch Logic for common kernels.}
  \label{fig:fusion}
\end{figure}




%matmul, mttkrp, repeated ttm, triangle counting, multiple pointwise,
%in-place.
%dot((v^t .* u), w)) vs. 
%(v^t .* dot(u, w))
